Optimal Learning Rates for Localized SVMs

One of the limiting factors of using support vector machines (SVMs) in large scale applications are their super-linear computational requirements in terms of the number of training samples. To address this issue, several approaches that train SVMs on many small chunks of large data sets separately have been proposed in the literature. So far, however, almost all these approaches have only been empirically investigated. In addition, their motivation was always based on computational requirements. In this work, we consider a localized SVM approach based upon a partition of the input space. For this local SVM, we derive a general oracle inequality. Then we apply this oracle inequality to least squares regression using Gaussian kernels and deduce local learning rates that are essentially minimax optimal under some standard smoothness assumptions on the regression function. This gives the first motivation for using local SVMs that is not based on computational requirements but on theoretical predictions on the generalization performance. We further introduce a data-dependent parameter selection method for our local SVM approach and show that this method achieves the same learning rates as before. Finally, we present some larger scale experiments for our localized SVM showing that it achieves essentially the same test performance as a global SVM for a fraction of the computational requirements. In addition, it turns out that the computational requirements for the local SVMs are similar to those of a vanilla random chunk approach, while the achieved test errors are significantly better.

==> macros2.tex <==
%----------------Used packages -------------------------

\usepackage[breaklinks=true]{hyperref}
\usepackage{breakurl}

\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{amsthm}
% \usepackage{textcmds}
\usepackage{dsfont}
\usepackage[latin1]{inputenc}
\usepackage{textcomp}
\usepackage{url}
\usepackage{framed}
\usepackage{graphics,overpic,color}
\usepackage{overpic}
\usepackage{color}
\usepackage[font=small]{caption}
\usepackage{wrapfig}
\usepackage[hang,footnotesize]{subfigure}
\usepackage[arrow, matrix, curve]{xy}
\usepackage{array} 
\usepackage{longtable}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{capt-of}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{rotfloat}
\usepackage{tikz}
\usetikzlibrary{matrix}
\usepackage{units}
\usepackage{paralist}
\usepackage[version-1-compatibility]{siunitx} 
%\usepackage[emulate=units]{siunitx} 


\newcommand{\RM}[1]{\MakeUppercase{\romannumeral #1}}

\definecolor{rot}{RGB}{255,0,0}
\definecolor{gruen}{RGB}{0,255,0}
\definecolor{blau}{RGB}{0,0,255}
\definecolor{violetred}{RGB}{208,32,144}


\DeclareSymbolFont{wideparensymbol}{OMX}{yhex}{m}{n}
\DeclareMathAccent{\wideparen}{\mathord}{wideparensymbol}{"F3}

% \DeclareSymbolFontAlphabet{\Bbb}{AMSb}


%---------------Theorem and friends-------------------------------------------------%

% 
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% 
% 
% %\theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% 
% \theoremstyle{definition}
% \newtheorem{example}[theorem]{Example}
% 
% 
% \theoremstyle{remark}
% \newtheorem{question}[theorem]{Question}
% \newtheorem{remark}[theorem]{Remark}
% 
% 
% \newcommand{\atob}[2]{\emph{#1)} $\Rightarrow$ \emph{#2)}.} 
% \newcommand{\ada}[1]{\emph{#1).}} 

%-------------tools----------------------------------


\newlength{\fixboxwidth}
\setlength{\fixboxwidth}{\marginparwidth}
\addtolength{\fixboxwidth}{-15pt}
\newcommand{\fix}[1]{\marginpar{%
    \fbox{\parbox{\fixboxwidth}{\tiny #1}}}}


%-------------paths-------------------------------


\newcommand{\bibtexpath}{}


%---------------Font switches -------------------------

\newcommand{\ca}[1]{{\cal #1}}


%----------------Formatting-----------------------------


\newcommand{\qspace}{\, , \qquad\qquad}
\renewcommand{\labelenumi}{\it\roman{enumi})}


%------------Fields and friends-------------------------------------------


\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rn}{\mathbb{R}^n}




%------------Expectations and friends-------------------------------------------

\newcommand{\E}{\mathbb{E}}


\newcommand{\EE}{\mathfrak{E}}

\newcommand{\Lt}{L_{\t}}
\newcommand{\ft}{f^*_{\t,\P}}
\newcommand{\Ft}{F^*_{\t,\P}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\Dbf}{\mathbf{D}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\fcl}{\wideparen{f}}
\newcommand{\fB}{f^*_{L,\P}}
\newcommand{\Lb}{\Lambda}
\newcommand{\Lbnj}{\Lb_{n,j}}
\newcommand{\lbnj}{\lb_{n,j}}
\newcommand{\fclip}[4]{\fcl_{#1_{#3,#4},#2_{#3,#4}}}
\newcommand{\f}[4]{f_{#1_{#3,#4},#2_{#3,#4}}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\cl}[1]{\wideparen{#1}}

\newcommand{\RLP}{\mathcal{R}_{L,\P}}
\newcommand{\RLtP}{\mathcal{R}_{L_{\t},\P}}
\newcommand{\RLPj}{\mathcal{R}_{L_{j},\P}}
\newcommand{\RLPJ}{\mathcal{R}_{L_J,\P}}
\newcommand{\RLPJT}{\mathcal{R}_{L_{J_T},\P}}
\newcommand{\RLPT}{\mathcal{R}_{L_{T},\P}}
\newcommand{\RLtPJT}{\mathcal{R}_{L_{\t,J_T},\P}}
\newcommand{\RLD}{\mathcal{R}_{L,\D}}
\newcommand{\RLDj}{\mathcal{R}_{L_{j},\D}}
\newcommand{\RLDJ}{\mathcal{R}_{L_J,\D}}
\newcommand{\RLDJT}{\mathcal{R}_{L_{J_T},\D}}
\newcommand{\RB}{\mathcal{R}_{L,\P}^*}
\newcommand{\RBj}{\mathcal{R}_{L_{j},\P}^*}
\newcommand{\RBJT}{\mathcal{R}_{L_{J_T},\P}^*}
\newcommand{\RBtJT}{\mathcal{R}_{L_{\t,J_T},\P}^*}
\newcommand{\RBJ}{\mathcal{R}_{L_J,\P}^*}
\newcommand{\RBT}{\mathcal{R}_{L_T,\P}^*}
\newcommand{\F}{\mathcal{F}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\eq}{\Longleftrightarrow}
\renewcommand{\L}{\mathcal{L}}

\newcommand{\bs}{\boldsymbol}
\newcommand{\TrP}[1]{{\P_X}_{|#1}}
\newcommand{\Cpp}{C\nolinebreak\hspace{-.05em}\raisebox{.4ex}{\tiny\bf +}\nolinebreak\hspace{-.10em}\raisebox{.4ex}{\tiny\bf +}}

\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg\,min}}}

%------------Greeks---------------------------------------------


\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\renewcommand{\d}{\delta}
% \newcommand{\D}{\Delta}
\newcommand{\e}{\varepsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\z}{\zeta}
\newcommand{\n}{\eta}
\newcommand{\vt}{\vartheta}
\renewcommand{\k}{\kappa}
\newcommand{\lb}{\lambda}
\newcommand{\x}{\xi}
\renewcommand{\r}{\rho}
\newcommand{\vr}{\varrho}
\newcommand{\s}{\sigma}
\newcommand{\vs}{\varsigma}
\renewcommand{\t}{\tau}
\newcommand{\p}{\varphi}
\renewcommand{\P}{\mathrm{P}}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\vU}{\varUpsilon}


%---------------Operators--------------------------------------

\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\spann}{span}
\DeclareMathOperator{\vol}{vol}
\newcommand{\radd}[1]{\mathrm{Rad}_{D}(#1)}
\newcommand{\radds}[1]{\mathrm{Rad}_{D'}(#1)}

%-----------------Operations and Relations --------------------------

\newcommand{\symdif}{\vartriangle}




%--------------Functions-----------------------------------

\DeclareMathOperator{\arcoth}{arcoth}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\sign}{sign}



%---------------Special Symbols------------------------------


\newcommand{\eins}{\boldsymbol{1}}
% \newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}} 



%---------------norms---------------------------------------

\newcommand{\snorm}[1]{\Vert #1 \Vert}
\newcommand{\mnorm}[1]{\bigl\Vert \, #1 \, \bigr\Vert}
\newcommand{\bnorm}[1]{\Bigl\Vert \, #1 \, \Bigr\Vert}
\newcommand{\lnorm}[1]{\biggl\Vert #1 \biggr\Vert}
\newcommand{\hnorm}[1]{\Vert #1 \Vert_{H}}
\newcommand{\inorm}[1]{\Vert #1 \Vert_\infty}




%---------------Risks and friends---------------------------------------

\newcommand{\RPo}[1]{{{\cal R}_{#1,\P}}}
\newcommand{\RTo}[1]{{{\cal R}_{#1,\mathrm{D}}}}
\newcommand{\RP}[2]{{{\cal R}_{#1,\P}(#2)}}
\newcommand{\RPB}[1]{{{\cal R}_{#1,\P}^{*}}}
\newcommand{\RT}[2]{{{\cal R}_{#1,\mathrm{D}}(#2)}}
\newcommand{\Rx}[3]{{{\cal R}_{#1,#2}(#3)}}
\newcommand{\Rxo}[2]{{{\cal R}_{#1,#2}}}
\newcommand{\RxB}[2]{{{\cal R}_{#1,#2}^*}}
\newcommand{\RxxB}[3]{{{\cal R}_{#1,#2,#3}^*}}
\newcommand{\RPxB}[2]{{{\cal R}_{#1,\P,#2}^*}}





%---------------diagrams---------------------------------------

\newcommand{\tridia}[6]{
\setlength{\unitlength}{1ex}
\begin{picture}(60,20)
\put(20,14){\makebox(9,2)[rt]{$#1$}}
\put(51,14){\makebox(9,2)[lt]{$#2$}}
\put(35.5,2){\makebox(9,2){$#3$}}
\put(30,15){\vector(1,0){20}}
\put(30,14){\vector(1,-1){9}}
\put(41,5){\vector(1,1){9}}
\put(37,16){\makebox(6,2){$#4$}}
\put(27.5,8){\makebox(6,2)[rt]{$#5$}}
\put(47.5,8){\makebox(6,2)[lt]{$#6$}}
\end{picture}}


\newcommand{\quadiasn}[8]{
\setlength{\unitlength}{1ex}
\begin{picture}(60,20)
\put(20,15){\makebox(9,2)[rt]{$#1$}}
\put(45,15){\makebox(9,2)[lt]{$#2$}}
\put(20,2){\makebox(9,2)[rt]{$#3$}}
\put(45,2){\makebox(9,2)[lt]{$#4$}}
\put(30,16){\vector(1,0){14}}
\put(25,14){\vector(0,-1){9}}
\put(49,5){\vector(0,1){9}}
\put(30,3){\vector(1,0){14}}
\put(34,17){\makebox(6,2){$#5$}}
\put(18,8.5){\makebox(6,2)[rt]{$#6$}}
\put(50,8.5){\makebox(6,2)[lt]{$#7$}}
\put(34,0){\makebox(6,2){$#8$}}
\end{picture}}



\newcommand{\quadiass}[8]{
\setlength{\unitlength}{1ex}
\begin{picture}(60,20)
\put(20,15){\makebox(9,2)[rt]{$#1$}}
\put(45,15){\makebox(9,2)[lt]{$#2$}}
\put(20,2){\makebox(9,2)[rt]{$#3$}}
\put(45,2){\makebox(9,2)[lt]{$#4$}}
\put(30,16){\vector(1,0){14}}
\put(25,14){\vector(0,-1){9}}
\put(49,14){\vector(0,-1){9}}
\put(30,3){\vector(1,0){14}}
\put(34,17){\makebox(6,2){$#5$}}
\put(18,8.5){\makebox(6,2)[rt]{$#6$}}
\put(50,8.5){\makebox(6,2)[lt]{$#7$}}
\put(34,0){\makebox(6,2){$#8$}}
\end{picture}}


\newcommand{\quadiann}[8]{
\setlength{\unitlength}{1ex}
\begin{picture}(60,20)
\put(20,15){\makebox(9,2)[rt]{$#1$}}
\put(45,15){\makebox(9,2)[lt]{$#2$}}
\put(20,2){\makebox(9,2)[rt]{$#3$}}
\put(45,2){\makebox(9,2)[lt]{$#4$}}
\put(30,16){\vector(1,0){14}}
\put(25,5){\vector(0,1){9}}
\put(49,5){\vector(0,1){9}}
\put(30,3){\vector(1,0){14}}
\put(34,17){\makebox(6,2){$#5$}}
\put(18,8.5){\makebox(6,2)[rt]{$#6$}}
\put(50,8.5){\makebox(6,2)[lt]{$#7$}}
\put(34,0){\makebox(6,2){$#8$}}
\end{picture}}

